Interpreting Low-level Vision Models with Causal Effect Maps

Deep neural networks have significantly improved the performance of low-level vision tasks but also increased the difficulty of interpretability. A deep understanding of deep models is beneficial for both network design and practical reliability. To take up this challenge, we introduce causality theory to interpret low-level vision models and propose a model-/task-agnostic method called Causal Effect Map (CEM). With CEM, we can visualize and quantify the input-output relationships on either positive or negative effects. After analyzing various low-level vision tasks with CEM, we have reached several interesting insights, such as: (1) Using more information of input images (e.g., larger receptive field) does NOT always yield positive outcomes. (2) Attempting to incorporate mechanisms with a global receptive field (e.g., channel attention) into image denoising may prove futile. (3) Integrating multiple tasks to train a general model could encourage the network to prioritize local information over global context. Based on the causal effect theory, the proposed diagnostic tool can refresh our common knowledge and bring a deeper understanding of low-level vision models. Codes are available at https://github.com/J-FHu/CEM.

==> figs/Exp1.tex <==

% \begin{figure*}[t] 
% \centering
%     \includegraphics[width=0.9\linewidth]{figs/sources/more_result_SR.pdf}
%     \caption{More CEM results of SR networks.}
%     \label{fig:Exp1}
% \end{figure*}


\begin{figure*}[htbp]
  \centering
  \rotatebox{90}{%
    \begin{minipage}{\textheight}
    \centering
\includegraphics[width=1\linewidth]{figs/sources/more_result_SR_modified.pdf}
    \caption{More CEM results of SR networks.}
    \label{fig:Exp1}
    \end{minipage}%
  }
\end{figure*}



==> figs/Exp2.tex <==

% \begin{figure}[htbp]
%   \centering
%   \rotatebox{90}{%
%     \begin{minipage}{\textheight}
%     \centering
% \includegraphics[width=1\linewidth]{figs/sources/more_result_SR_modified.pdf}
%     \caption{More CEM results of SR networks.}
%     \label{fig:Exp1}
%     \end{minipage}%
%   }
% \end{figure}


\begin{figure*}[htbp]
  \centering
  \rotatebox{90}{%
    \begin{minipage}{\textheight}
    \centering
    \includegraphics[width=0.85\linewidth]{figs/sources/more_result_DN_modified.pdf}
    \caption{More CEM results of DN networks.}
    \label{fig:Exp2}
    \end{minipage}%
  }
\end{figure*}

==> figs/Exp3.tex <==
\begin{figure*}[htbp]
  \centering
  \rotatebox{90}{%
    \begin{minipage}{\textheight}
    \centering
    \includegraphics[width=0.89\linewidth]{figs/sources/more_result_DR_modified.pdf}
    \caption{More CEM results of DR networks.}
    \label{fig:Exp3}
    \end{minipage}%
  }
\end{figure*}

==> figs/correlation.tex <==
\begin{figure}[tpb]
    \centering
    \includegraphics[width=\linewidth]{figs/sources/corr_cau.pdf}
    \caption{
    (a) Correlations between \textit{a}, \textit{b}, \textit{c} and \textit{R}, $\mathcal{M}_\textit{R}$ denotes some kind of measurement for \textit{R}.
    %
    Intervening in \textit{a} ($\textit{do}(a=x)$), \textit{b} ($\textit{do}(b=x)$), and \textit{c} ($\textit{do}(c=x)$) reveals that (b) variable \textit{a} has no causal relationship with \textit{R}, (c) variable \textit{b} has a negative causal effect, while (d) variable \textit{c} has a positive causal effect.
    %
    The black undirected edge represents two variables that correlate. The blue-directed and red-directed edges show the negative and positive causal relationship, respectively.
    %
    (e) Examining the relationship between input patches \textit{a}, \textit{b}, \textit{c} and the reconstruction of ROI \textit{R}.
    %
    (f) The LAM of RNAN, red dots represent the correlation. (g) The CEM of RNAN, patches with negative and positive effect are highlighted in blue and red.
    }
    \label{fig:correlation}
\end{figure}


==> table/table1.tex <==
\begin{table*}
\label{tab:1}
    \centering\renewcommand\arraystretch{1}\setlength{\tabcolsep}{6pt}
    % \hspace{-4mm}
    % \small
    \begin{tabular}{lccc}
                \Xhline{1.2pt}
                Mechanism & Super-Resolution & Denoise & Derain\\
                \Xhline{1.2pt}
                CNN & \makecell[c]{SRCNN, EDSR\\CARN, SRDenseNet, SRResNet} & \makecell[c]{FFDNet, DnCNN\\SADNet, SRResNet} & PReNet, HINet, SRResNet  \\ 
                \Xhline{0.01pt}
                Global Attention  & DRLN, RNAN, SAN, RCAN & RCAN, MPRNet & RCAN, MPRNet  \\ 
                \Xhline{0.01pt}
                Transformer   & SwinIR, HAT,  XRestormer & SCUNet, SwinIR,XRestormer  & SwinIR, XRestormer  \\
                \Xhline{1.2pt}
  \end{tabular}
    % \vspace{-3mm}
    \caption{The involved LV tasks and models in our experiments.}
    \vspace{-4mm}
\end{table*}
